Leveraging Mixture of Experts for Improved Speech Deepfake Detection

Speech deepfakes pose a significant threat to personal security and content authenticity. Several detectors have been proposed in the literature, and one of the primary challenges these systems have to face is the generalization over unseen data to identify fake signals across a wide range of datasets. In this paper, we introduce a novel approach for enhancing speech deepfake detection performance using a Mixture of Experts architecture. The Mixture of Experts framework is well-suited for the speech deepfake detection task due to its ability to specialize in different input types and handle data variability efficiently. This approach offers superior generalization and adaptability to unseen data compared to traditional single models or ensemble methods. Additionally, its modular structure supports scalable updates, making it more flexible in managing the evolving complexity of deepfake techniques while maintaining high detection accuracy. We propose an efficient, lightweight gating mechanism to dynamically assign expert weights for each input, optimizing detection performance. Experimental results across multiple datasets demonstrate the effectiveness and potential of our proposed approach.

==> 2_method_old.tex <==
\glsreset{moe}

\section{Proposed Method}
\label{sec:method}

In this section, we formalize the task at hand, i.e., speech deepfake detection, and present an outline of our proposed approach based on a \gls{moe} framework.

\subsection{Problem Formulation}
\label{subsec:problem}

The speech deepfake detection problem is formally defined as follows.
Let us consider a discrete-time input speech signal $\mathbf{x}$ sampled at a frequency $f_\text{s}$ and associated with a class $y \in \{0, 1\}$, where \num{0} denotes that the signal is authentic and \num{1} indicates that it has been synthetically generated.
The goal of this task is to develop a detector $\mathcal{D}$ that estimates the class of the signal $\mathbf{x}$ as $\hat{y} \in [0,1]$, where $\hat{y}$ is 
the likelihood of the signal $\mathbf{x}$ being fake.
% The detector $\mathcal{D}$ can be implemented in different ways. Among the most common approaches, we can train it in an end-to-end fashion or consider it as a combination of a feature extractor and a classifier.
 
\subsection{Proposed Systems}
\label{subsec:system}

In the proposed approach, we design the detector $\mathcal{D}$ as a \gls{moe} specifically tailored for the speech deepfake detection task.
Our \gls{moe} system is composed of multiple detectors, each pre-trained on a different speech deepfake dataset, thus becoming an ``expert'' in that domain. 
We denote the $i$-th expert as $\mathcal{E}_i$, where $i \in \{1, 2, \ldots, N\}$, and $N$ represents the total number of considered domains.
%The core of the \gls{moe} framework is the gating network $\mathcal{G}$. %, which is responsible for routing the input $\mathbf{x}$ to the appropriate expert.
While all experts are fed with the same audio signal $\mathbf{x}$, the input of the gating network $\mathcal{G}$ varies based on the chosen \gls{moe} implementation.

We consider two different architectures for the \gls{moe} framework, which we will later refer to as \textit{standard} and \textit{enhanced}, respectively. 
These are both \textit{dense} \glspl{moe}, meaning that every expert $\mathcal{E}_i$ is queried for each input $\mathbf{x}$~\cite{cai2024survey}. 
The standard model is a classic \gls{moe} inspired by \cite{jacobs1991adaptive},  
where both $\mathcal{G}$ and the experts $\mathcal{E}_i$ directly receive the input audio excerpt $\mathbf{x}$.
%equipped with a gating that does not rely on the internal representation of the experts to compute expert weights but solely on the input $\mathbf{x}$.
%The gating network of the second \gls{moe}, in contrast, takes as input concatenated embeddings from each expert, along with a combined embedding created through a learnable weighted element-wise multiplication of the individual embeddings.
The enhanced \gls{moe} architecture features a gating network $\mathcal{G}$ that relies on the internal representations produced by the $N$ experts.
In this design, the gating network uses the first few layers of the experts as embedding extractors and takes as input a concatenation of the embeddings from each expert, along with a combined embedding. Each expert embedding $\mathbf{e}_\text{i}\in\mathbb{R}^d$ is extracted from the last batch normalization layer of $\mathcal{E}_i$.
The combined embedding $\mathbf{w}\in\mathbb{R}^d$, in turn, is created through a learnable weighted element-wise multiplication of $\mathbf{e}_\text{1}, ..., \mathbf{e}_\text{N}$.
%Let $\mathbf{e}_\text{i}$ denote the embedding output from expert $\mathcal{E}_\text{i}$ for the given input $\mathbf{x}$, as in $\mathbf{e}_\text{i} =\mathcal{E}_\text{i}(\mathbf{x})$. 
%Each embedding $\mathbf{e}_\text{i}$ is a vector in $\mathbb{R}^{d}$, where $d$ is the dimensionality of the embedding space. 
Considering $N=4$ and $d=64$, the combined embedding is calculated as:
\begin{equation}
\mathbf{w} = (\mathbf{e}_1 \odot \mathbf{e}_2 \odot \mathbf{e}_3 \odot \mathbf{e}_4) \odot \mathbf{p}, 
\end{equation}
where $\odot$ denotes element-wise multiplication, and $\mathbf{p} \in \mathbb{R}^{d}$ is a learnable parameter.
The final concatenated embedding vector $\mathbf{e}_{\text{input}}$ is formed by:
\begin{equation}
\mathbf{e}_{\text{input}} = [\mathbf{e}_1, \mathbf{e}_2, \mathbf{e}_3, \mathbf{e}_4, \mathbf{w}],
\label{eq:input_gating}
\end{equation}
where $[\cdot]$ denotes vector concatenation. 
This specific design is intended to fully leverage the domain-specific knowledge acquired during pre-training to enhance the overall performance.
We draw inspiration for this approach from~\cite{lee2014speaker}.

In both architectures, the gating network produces a set of weights for each expert.
The output logits of the \glspl{moe} systems are a weighted sum of the output logits from all experts, as in:
\begin{equation}
    \mathbf{z} = \sum_{\text{i}=1}^N \alpha_\text{i}(\mathbf{x}) \cdot \mathcal{E}_\text{i}(\mathbf{x}),
    \label{eq:w_average}
\end{equation}
where $\alpha_\text{i}(\mathbf{x})$ represents the gating weight for expert $\mathcal{E}_\text{i}$ given the input $\mathbf{x}$, and $\mathcal{E}_\text{i}(\mathbf{x})$ is the output of expert $\mathcal{E}_\text{i}$. 
This approach is known as \textit{soft} \gls{moe}~\cite{cai2024survey}, as it employs soft weights rather than hard, discrete activations.
The final prediction score $\hat{y}$ of the complete speech deepfake detector $\mathcal{D}$ is obtained by applying a softmax function to the weighted logits vector $\mathbf{z}$. %:
%\begin{equation}
%    \hat{y} = \text{softmax}(\mathbf{z}),
%\end{equation}
%where $\hat{y}$ represents the soft score for input $\mathbf{x}$. 
%The final decision is made by thresholding the positive class probability to determine whether the input is genuine or fake. 

